Context-Aware Aerial Object Detection: Leveraging Inter-Object and Background Relationships

In most modern object detection pipelines, the detection proposals are processed independently given the feature map. Therefore, they overlook the underlying relationships between objects and the surrounding background, which could have provided additional context for accurate detection. Because aerial imagery is almost orthographic, the spatial relations in image space closely align with those in the physical world, and inter-object and object-background relationships become particularly significant. To address this oversight, we propose a framework that leverages the strengths of Transformer-based models and Contrastive Language-Image Pre-training (CLIP) features to capture such relationships. Specifically, Building on two-stage detectors, we treat Region of Interest (RoI) proposals as tokens, accompanied by CLIP Tokens obtained from multi-level image segments. These tokens are then passed through a Transformer encoder, where specific spatial and geometric relations are incorporated into the attention weights, which are adaptively modulated and regularized. Additionally, we introduce self-supervised constraints on CLIP Tokens to ensure consistency. Extensive experiments on three benchmark datasets demonstrate that our approach achieves consistent improvements, setting new state-of-the-art results with increases of 1.37 mAP$_{50}$ on DOTA-v1.0, 5.30 mAP$_{50}$ on DOTA-v1.5, 2.30 mAP$_{50}$ on DOTA-v2.0 and 3.23 mAP$_{50}$ on DIOR-R.

==> table_backup/ab3_select_rpe.tex <==
\begin{table}[h]
\centering
\caption{}
\label{tab:ab_attention}
\begin{tabular}{c|c}
\toprule
Attention Weights ($\beta$)   & mAP   \\ \hline
baseline (ReDet)    & 66.86 \\
\specialtext{fixed scaling ($\epsilon=\sqrt{S}=32$)}       & 70.35(+3.49) \\
\specialtext{no duplicate masking}    & 67.32(+0.46) \\
\specialtext{no density ($\bar{\rho}_i=0$)} & 69.85(+2.99) \\
Ours        & 71.74(+4.88) \\ \bottomrule
\end{tabular}
\end{table}

==> table_backup/ab4_diff_formula.tex <==
\begin{table}[h]
\centering
\caption{Choice of attention functions.}
\label{ab4}
\begin{tabular}{c|c}
\hline
Formula & mAP \\ \hline
$\exp{(-(\epsilon d))}$ & 69.02 \\
$1/(1+\epsilon d)$ & 71.24 \\
$[1/(1+\epsilon d)]^2$ & 70.27 \\
$\exp{(-(\epsilon d)^2/2\sigma ^ 2)}$ & 71.74 \\ \hline
\end{tabular}
\end{table}

==> table_backup/ablation9.tex <==
% \begin{table}[]
% \centering

% \begin{minipage}{0.36\textwidth}
% \centering
% \caption{Detection performance with and without self-supervised loss.}
% \label{tab:ab_self_super}
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c}
%     \toprule
%     Self supervised loss & mAP   \\ \hline
%     w/o       & 71.89 \\
%     w         & 72.16 \\ \bottomrule
%     \end{tabular}
% }
% % \begin{tabular}{c|c}
% %     \toprule
% %     pre cls supervision & mAP   \\ \hline
% %     w/o       & 69.86 \\
% %     w         & \highlight{71.74} \\ \bottomrule
% % \end{tabular}
% \end{minipage} 
% % \hfill
% % \hspace{10pt}
% \centering

% \begin{minipage}{0.36\textwidth}
% \centering
% \caption{Detection performance with and without multi-level fusion.}
% \label{tab:ab_multi_level}
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c}
%     \toprule
%     Multi-level fusion & mAP   \\ \hline
%     w/o       & 71.17 \\
%     w         & 72.16 \\ \bottomrule
%     \end{tabular}
% }
% \end{minipage} 
% \vspace{5pt}
% \end{table}

\begin{table}[]
\centering

\begin{minipage}{0.36\textwidth}
\centering
\caption{Detection performance with and without self-supervised loss.}
\label{tab:ab_self_super}
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|c}
    \toprule
    Self supervised loss & mAP   \\ \hline
    w/o       & 71.89 \\
    w         & 72.16 \\ \bottomrule
    \end{tabular}
}
% \begin{tabular}{c|c}
%     \toprule
%     pre cls supervision & mAP   \\ \hline
%     w/o       & 69.86 \\
%     w         & \highlight{71.74} \\ \bottomrule
% \end{tabular}
\end{minipage} 
% \hfill
\hspace{20pt}
\begin{minipage}{0.36\textwidth}
\centering
\caption{Detection performance with and without multi-level fusion.}
\label{tab:ab_multi_level}
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|c}
    \toprule
    Multi-level fusion & mAP   \\ \hline
    w/o       & 71.17 \\
    w         & 72.16 \\ \bottomrule
    \end{tabular}
}

\end{minipage}

\vspace{5pt}
\end{table}

==> table_backup/ablation_eq8.tex <==
\begin{table}[]
\centering

\begin{minipage}{0.36\textwidth}
\centering
\caption{Detection performance with and without preliminary detection training.}
\label{tab:ab_pre_cls}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c}
    \toprule
    pre cls supervision & mAP   \\ \hline
    w/o       & 69.86 \\
    w         & 71.74 \\ \bottomrule
    \end{tabular}
}
% \begin{tabular}{c|c}
%     \toprule
%     pre cls supervision & mAP   \\ \hline
%     w/o       & 69.86 \\
%     w         & \highlight{71.74} \\ \bottomrule
% \end{tabular}
\end{minipage} 
% \hfill
\hspace{10pt}
\begin{minipage}{0.48\textwidth}
\centering
\caption{Effect of the components in computing the attention weights via \cref{eq:weights}. Relations are calculated in \cref{eq:P}, and Adaptive weight is calculated in \cref{eq:beta}}
\label{tab:ab_attention}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{cccc|c}
    \toprule
    RoI Tokens &  CLIP Tokens & Relations & Ada. Weight & mAP \\ \midrule
                &            &           &           & 66.86 \\
    \checkmark  &            &           &           & 69.02 \\
    \checkmark  & \checkmark &           &           & 70.96\\
    \checkmark  & \checkmark &  \checkmark &         & 70.87 \\
    \checkmark  & \checkmark &            &\checkmark & 71.61 \\ 
    \checkmark  & \checkmark & \checkmark &\checkmark & 72.16 \\ \bottomrule
    \end{tabular}
}
% \begin{tabular}{ccc|c}
%     \toprule
%     Transformer & Relations ($P$) & Ada. Weight ($\beta$) & mAP \\ \midrule
%                 &            &            & 66.86 \\
%     \checkmark  &            &            & 69.02 \\
%     \checkmark  & \checkmark &            & 71.09 \\
%     \checkmark  &            & \checkmark & 70.87 \\
%     \checkmark  & \checkmark & \checkmark & 71.74 \\ \bottomrule
% \end{tabular}
\end{minipage}
\vspace{5pt}
\end{table}

==> table_backup/different_model.tex <==
\begin{table}[]
\caption{More experiments on DOTA-v1.5. We highlight our method's improvements in \highlight{blue}}.

\centering
\label{tab:diff_method}
\begin{tabular}{l|c}
\toprule
Method                     & mAP   \\ \hline
RoI Transformer                  & 66.69 \\
RoI Transformer + Ours           & \highlight{68.69(+2.00)} \\\hline
% Oriented RCNN              & 65.94 \\
% Oriented RCNN + Ours       & \highlight{66.38(+0.44)} \\\hline
Rotated Faster RCNN        & 64.63 \\
Rotated Faster RCNN + Ours & \highlight{65.28(+0.65)} \\\hline
ReDet                      & 66.86 \\
Ours (ReDet)               & \highlight{72.16(+5.30)} \\
\bottomrule
\end{tabular}
\end{table}

==> table_backup/dotav10.tex <==
\begin{table}[]
\centering
\caption{Results on DOTA-v1.0. }
\label{tab:dota-v1.0}
% \begin{tabular}{l|p{1.51cm}llp{1.51cm}l}
\begin{tabular}{l|l|lll}
\toprule
Method  & AP50         & AP75         & mAP          \\ \hline
ReDet & 76.25        & 50.86        & 47.11        \\
Ours     & \highlight{77.84(+1.59)} & \highlight{51.42(+0.56)} & \highlight{48.32(+1.21)} \\ \bottomrule
\end{tabular}
\end{table}

==> table_backup/hrsc2016.tex <==
\begin{table}[h]
\centering
\caption{Ablation of the relations considered for computing the attention weights.}
\label{tab:ab_relations}
\begin{tabular}{cccccc|c}
\toprule
$dx$         & $dy$         & $d\alpha$   & dist       & IoU         & area  & mAP \\ \hline
           &            &            &            &             &            & 70.87   \\
\checkmark & \checkmark & \checkmark &            &             &             & 70.87  \\
\checkmark & \checkmark & \checkmark & \checkmark &             &             & 70.96  \\
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark &            & 71.51 \\
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  71.74 \\ \bottomrule
\end{tabular}
\end{table}

==> table_backup/table6_7.tex <==
\begin{table}[ht]
    \caption{Design choices of the relations and adaptive weights.}
    % \vspace{-10pt}
    \centering
    \begin{subtable}{.45\linewidth}
        \caption{Effect of the spatial and geometric relations.}
        \centering

        \begin{tabular}{@{}p{3cm}c@{}}
            \toprule
            \multicolumn{1}{c}{Method} & mAP   \\ \midrule
            % None                       & 70.41 \\
            $dx$ $dy$                  & 70.79 \\
            \ \  + $da$  dist                   & 71.03 \\
            \ \ \ \ + IoU                  & 71.46 \\
            \ \ \ \ \ \ \ \ + area               & 72.16 \\ \bottomrule
        \end{tabular}

        % \begin{tabular}{cccccc|c}
        % \toprule
        % $dx$         & $dy$         & $d\alpha$   & dist       & IoU         & area  & mAP \\ \hline
        %            &            &            &            &             &            & 70.87   \\
        % \checkmark & \checkmark & \checkmark &            &             &             & 70.87  \\
        % \checkmark & \checkmark & \checkmark & \checkmark &             &             & 70.96  \\
        % \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &            & 71.51 \\
        % \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  71.74 \\ \bottomrule
        % \end{tabular}
        \label{tab:ab_relations}
    \end{subtable}%
    \hfill
    \begin{subtable}{.45\linewidth}
        \caption{Effect of the factors in computing $\beta$.}
        \centering
        \begin{tabular}{c|c}
        \toprule
        Attention Weights ($\beta$)   & mAP   \\ \hline
        baseline (ReDet)    & 66.86 \\
        \specialtext{- scale ($\epsilon=\sqrt{S}=32$)}       & 70.49 \\
        % \specialtext{- overlap ($\delta=1$)}    & 67.32 \\
        \specialtext{- density ($\bar{\rho}_i=0$)} & 71.30 \\
        Ours        & 72.16 \\ \bottomrule
        \end{tabular}
        \label{tab:ab_adaptive}
    \end{subtable}
    % \label{tab:both_tables}
\end{table}

==> table_backup/table_main_and_pre_cls.tex <==
\begin{table*}[ht]
\centering
\begin{minipage}{0.68\textwidth}
\centering
\caption{mAP$_{50}$ results on DOTA-v1.0/v1.5/v2.0, and DIOR-R. For DOTA-v2.0, we use Oriented R-CNN as the baseline due to out-of-memory issues with the original ReDet. For the other datasets, ReDet is used as the baseline. We highlight our method's improvements in \highlight{blue}.}
% \small
\begin{tabular}{l|llll}
\toprule
Method        & DOTA-v1.0 & DOTA-v1.5 & DOTA-v2.0 & DIOR-R \\ \hline
Baseline      & 76.25     & 66.86     & 53.28     & 65.79  \\
Baseline+Ours & 77.62\highlight{(+1.37)}     & 72.16\highlight{(+5.30)}    & 55.58\highlight{(+2.30)}     & 69.02\highlight{(+3.23)}  \\ \bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.28\textwidth}
\centering
\caption{Detection performance with and without preliminary detection training.}
\label{tab:ab_pre_cls}
\begin{tabular}{c|c}
\toprule
pre cls supervision & mAP   \\ \hline
w/o       & 69.86 \\
w         & 71.74 \\ \bottomrule
\end{tabular}
\end{minipage}
\end{table*}


==> table_backup/tables_main_and_two.tex <==
\begin{table*}[ht]
\centering
% 左边的大表格
\begin{minipage}{0.6\textwidth}
\centering
\begin{tabular}{l|l|lll}
\toprule
Dataset  &        Method            & AP50         & AP75         & mAP          \\ \hline
\multirow{2}{*}{DOTA-v1.0} & ReDet  & 76.25        & 50.86        & 47.11        \\
   &        Ours                    & 77.62\highlight{(+1.37)} & 52.18\highlight{(+1.32)} & 48.67\highlight{(+1.56)} \\ \hline
\multirow{2}{*}{HRSC2016}  & ReDet  & 90.46        & 89.46        & 70.41        \\
   &        Ours                    & 90.49\highlight{(+0.03)} & 89.67\highlight{(+0.21)} & 72.51\highlight{(+2.10)} \\ \bottomrule
\end{tabular}
\caption{Results in COCO style on DOTA-v1.0 and HRSC2016. We highlight our method's improvements in \highlight{blue}.}
\label{tab:results2}
\end{minipage}
% \hfill
% 右边的小表格（上下排列）
\quad



% \begin{minipage}{0.3\textwidth}
% \centering
% \label{tab:ab_self_super}
% \begin{tabular}{c|c}
% \toprule
% Self supervised loss & mAP   \\ \hline
% w/o       & 71.89 \\
% w         & 72.16 \\ \bottomrule
% \end{tabular}
% \caption{Detection performance with and without self-supervised loss.}
% % \vspace{1em}  % 添加垂直间
% \centering
% \label{tab:ab_multi_level}
% \begin{tabular}{c|c}
% \toprule
% Multi-level fusion & mAP   \\ \hline
% w/o       & 71.17 \\
% w         & 72.16 \\ \bottomrule
% \end{tabular}
% \caption{Detection performance with and without multi-level fusion.}
% \end{minipage}



\begin{minipage}{0.3\textwidth}
\begin{tabular}{cll}
Module                                                                           & w w/o & \textbackslash{}text\{mAP\}\%\_50\% \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Self supervised \\ loss\end{tabular}} & w     & 71.89                               \\
                                                                                 & w/o   & 72.16                               \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Multi-level \\ fusion\end{tabular}}   & w     & 71.17                               \\
                                                                                 & w/o   & 72.16                              
\end{tabular}
\end{minipage}



\end{table*}

